Gistable: Evaluating the Executability of Python Code Snippets on GitHub

Software developers create and share code online to demonstrate programming language concepts and programming tasks. Code snippets can be a useful way to explain and demonstrate a programming concept, but may not always be directly executable. A code snippet can contain parse errors, or fail to execute if the environment contains unmet dependencies. This paper presents an empirical analysis of the executable status of Python code snippets shared through the GitHub gist system, and the ability of developers familiar with software configuration to correctly configure and run them. We find that 75.6% of gists require non-trivial configuration to overcome missing dependencies, configuration files, reliance on a specific operating system, or some other environment configuration. Our study also suggests the natural assumption developers make about resource names when resolving configuration errors is correct less than half the time. We also present Gistable, a database and extensible framework built on GitHub's gist system, which provides executable code snippets to enable reproducible studies in software engineering. Gistable contains 10,259 code snippets, approximately 5,000 with a Dockerfile to configure and execute them without import error. Gistable is publicly available at https://github.com/gistable/gistable.

==> tables/tbl-characteristics.tex <==
\begin{table*}
    \begin{center}
        \begin{threeparttable}
            \caption{
                We analyzed an additional 30 random gists to define environment characteristics related
                to execution failure. Some gists have multiple characteristics which may prevent
                them from exiting with \texttt{Success}.
                \todo{Why doesn't this add up to 30?}
                \todo{Inline this}
            }
            \label{tbl:characteristics}
            \begin{tabulary}{\textwidth}{p{0.5\textwidth}p{0.05\textwidth}p{0.35\textwidth}}
                \toprule
                \textbf{Cause} & \textbf{Count}  & \textbf{Example} \\ 
                \midrule
                
                Relies on network resources &
                    10 & \url{https://gist.github.com/bkjones/1902478} \\ \midrule
                Relies on a resource being present at a specific location on the filesystem &
                    10 & \url{https://gist.github.com/EderSantana/5a5c3a6ad327f303cb915198aec8a90d} \\ \midrule
                Relies on a graphics display &
                    3 & \url{https://gist.github.com/kriben/1410088} \\
                    
                \bottomrule
            \end{tabulary}
            % \begin{tablenotes}
            %     \item[1] Note
            % \end{tablenotes}
        \end{threeparttable}
    \end{center}
\end{table*}

